Learning Deep Structure-Preserving Image-Text Embeddings

This paper proposes a method for learning joint embeddings of images and text using a two-branch neural network with multiple layers of linear projections followed by nonlinearities. The network is trained using a large margin objective that combines cross-view ranking constraints with within-view neighborhood structure preservation constraints inspired by metric learning literature. Extensive experiments show that our approach gains significant improvements in accuracy for image-to-text and text-to-image retrieval. Our method achieves new state-of-the-art results on the Flickr30K and MSCOCO image-sentence datasets and shows promise on the new task of phrase localization on the Flickr30K Entities dataset.

==> weighted_distance.tex <==

\begin{table*}[h]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
Methods on Flickr30K & \multicolumn{3}{l|}{Image-to-sentence} & \multicolumn{3}{l|}{Sentence-to-image} \\ \hline
  & R@1            & R@5            & R@10          & R@1            & R@5            & R@10          \\ \hline
 Nonlinear + bi-directional + structure   & 40.3   &  68.9    & 79.9      &  29.7    &  60.1   & 72.1      \\ 
Weighted distance  &  40.9   &  69.5    & 80.5      &  30.2    &  60.8   & 72.6   \\ \hline
% Fine-tuned weighted distance  &  \textbf{41.6}   &  \textbf{70.5}    & \textbf{81.0}      &  \textbf{30.8}    &  \textbf{61.1}   & \textbf{73.3} \\ \hline
\end{tabular}
\caption{Results on Flickr30K image-sentence retrieval by incorporating region-phrase correspondences (see text).}
\label{table:weighted}
\end{table*}

\subsection{Weighted Image-Sentence Embedding}

Finally, we investigate how the region-phrase embedding learned in Section \ref{sec_rp} can help with global image-sentence retrieval. To modify our learning framework, in the embedding loss layer, we redefine the distance $D(x,y)$ between image $x$ and sentence $y$ to be the following:

\begin{equation}\label{eq:weighted}
D(x,y) = (1-\alpha)\,d(x,y) + \alpha \,d_{rp}(x,y) \,,
\end{equation}

\noindent where $d(x,y)$ is the distance in the image-sentence embedding space, and $d_{rp}(x,y)$ is defined as the average of the distances between the phrases in the sentence and their best-matching regions in the image. This is referred to as {\em weighted distance} in~\cite{plummer2015flickr30k}.
%with $d_{rp}(x,y) = \sum_{i=1}^P f_{rp}(x)^T g_{rp}(y)$. In \cite{plummer2015flickr30k}, this is named as a \textit{weighted distance} between x and y. 

% \begin{table*}[b]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% Methods on Flickr30K & \multicolumn{3}{l|}{Image-to-sentence} & \multicolumn{3}{l|}{Sentence-to-image} \\ \hline
%   & R@1            & R@5            & R@10          & R@1            & R@5            & R@10          \\ \hline
%  Nonlinear + bi-directional + structure   &  41.5   &  70.4    & 80.5      &  29.4    &  60.4   & 72.6      \\ 
% Weighted distance  &  \textbf{42.0}   &  \textbf{71.4}    & \textbf{81.8}      &  \textbf{30.2}    &  \textbf{61.6}   & \textbf{73.2}   \\ 
% Fine-tuned weighted distance  &  \textbf{42.8}   &  \textbf{72.1}    & \textbf{82.7}      &  \textbf{31.5}    &  \textbf{62.4}   & \textbf{74.2} \\ \hline
% \end{tabular}
% \caption{Results on Flickr30K image-sentence retrieval by incorporating region-phrase correspondences (see text).}
% \label{table:weighted}
% \end{table*}


The second line of Table \ref{table:weighted} gives the result of using weighted distance at test time with separately trained image-sentence and region-phrase embedding networks (we choose $\alpha=0.7$ following \cite{plummer2015flickr30k}). By comparing with the first line of Table \ref{table:weighted}, which repeats our best global image-sentence result from Table \ref{table:flickr30k}, we can see that we get an improvement of 0.5-1\%, which is consistent with the small improvements reported in~\cite{plummer2015flickr30k} from adding region-phrase correspondence at test time. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Next, we are interested in whether we can use the region-phrase embedding to fine-tune the image-sentence network. We start with image-sentence and region-phrase networks pre-trained for 30 epochs. During the fine-tuning, in the top embedding loss layer, we calculate the weighted distance (eq. \ref{eq:weighted}) and back-propagate it to update the parameters of the image-sentence network for another 3 epochs. The last line of Table \ref{table:weighted} shows that this fine-tuning gives another 0.5-1\improvement on image-sentence retrieval. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%given one image-sentence pair, for the image-sentence networks, we still pass into the random splited mini-batch pairs, while for the region-phrase embedding networks, we pass the corresponding region-phrases pairs that are parts of the image-sentence pairs. But different from training the independent region-phrase networks in sec.(\ref{sec_rp}) that uses ground-truth pairs, here, we use the automatically parsed phrases (from those sentences in the mini-batch) and max covered region (compared with ground-truth region) as the mini-batch to the region-phrase networks. In the top embedding loss layer, we calculate the region-phrase distance $d_{r}(x,y) = \sum_{i=1}^P f_{rp}(x)^T g_{rp}(y)$ and have the averaged region-phrase distance. Then, we do back-propagation to image-sentence networks and update its parameters based on the newly accumulated gradients calculated from Eq.(\ref{eq:weighted}). For region-phrases networks, we update its parameters independently. 

%In testing, given one image and sentence pair, for each phrase feature $g_{rp}(y)$ automatically generated from the sentence, we obtain the top-ranked candidate region $f_{rp}(y)$ from the 100 proposals in the testing image. Then we compute the distance $d_{rp}$ between the sentence defined as a set of phrases and the image defined as the set of regions. At the same time, we pass the image and sentence pair to the image-sentence embedding and calculate the weighted distance by Eq.(\ref{eq:obj}). For fair comparison, during the fine-tuning, we also use the same value $\alpha = 0.7$. Experiments in Table.(\ref{table:weighted}) shows that, this fine-tuned weighted distance gives better performance than calculating them separately.


% \begin{table*}
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% Methods on Flickr30K & \multicolumn{3}{l|}{Image-to-sentence} & \multicolumn{3}{l|}{Sentence-to-image} \\ \hline
%   & R@1            & R@5            & R@10          & R@1            & R@5            & R@10          \\ \hline
%  Nonlinear + bi-directional + structure   &  41.5   &  70.4    & 80.5      &  29.4    &  60.4   & 72.6      \\ 
% Weighted distance  &  \textbf{42.0}   &  \textbf{71.4}    & \textbf{81.8}      &  \textbf{30.2}    &  \textbf{61.6}   & \textbf{73.2}   \\ 
% Fine-tuned weighted distance  &  \textbf{42.8}   &  \textbf{72.1}    & \textbf{82.7}      &  \textbf{31.5}    &  \textbf{62.4}   & \textbf{74.2} \\ \hline
% \end{tabular}
% \caption{Results on Flickr30K image-sentence retrieval by incorporating region-phrase correspondences (see text).}
% \label{table:weighted}
% \end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We are currently working on better methods for jointly fine-tuning the image-sentence and region-phrase networks. In the meantime, we can observe that our preliminary approach of replacing the image-sentence distance $d(x,y)$ in eq. (\ref{eq:obj}) by the weighted distance (eq. \ref{eq:weighted}) has the effect of modifying the margin $m$ by the region-phrase distance on a per-instance basis. Scaling the margin is a standard technique in the structured learning literature~\cite{joachims2009cutting}, and we plan to explore more powerful applications of this idea to obtain bigger improvements. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[h]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% Methods on Flickr30K & \multicolumn{3}{l|}{Image-to-sentence} & \multicolumn{3}{l|}{Sentence-to-image} \\ \hline
%   & R@1            & R@5            & R@10          & R@1            & R@5            & R@10          \\ \hline
%  Nonlinear + bi-directional + structure   &  41.5   &  70.4    & 80.5      &  29.4    &  60.4   & 72.6      \\ 
% Weighted distance  &  \textbf{42.0}   &  \textbf{71.4}    & \textbf{81.8}      &  \textbf{30.2}    &  \textbf{61.6}   & \textbf{73.2}   \\ 
% Fine-tuned weighted distance  &  \textbf{42.8}   &  \textbf{72.1}    & \textbf{82.7}      &  \textbf{31.5}    &  \textbf{62.4}   & \textbf{74.2} \\ \hline
% \end{tabular}
% \caption{Results on Flickr30K image-sentence retrieval by incorporating region-phrase correspondences (see text).}
% \label{table:weighted}
% \end{table*}












